DreamInpainter: Text-Guided Subject-Driven Image Inpainting with Diffusion Models

This study introduces Text-Guided Subject-Driven Image Inpainting, a novel task that combines text and exemplar images for image inpainting. While both text and exemplar images have been used independently in previous efforts, their combined utilization remains unexplored. Simultaneously accommodating both conditions poses a significant challenge due to the inherent balance required between editability and subject fidelity. To tackle this challenge, we propose a two-step approach DreamInpainter. First, we compute dense subject features to ensure accurate subject replication. Then, we employ a discriminative token selection module to eliminate redundant subject details, preserving the subject's identity while allowing changes according to other conditions such as mask shape and text prompts. Additionally, we introduce a decoupling regularization technique to enhance text control in the presence of exemplar images. Our extensive experiments demonstrate the superior performance of our method in terms of visual quality, identity preservation, and text control, showcasing its effectiveness in the context of text-guided subject-driven image inpainting.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}



% \kelvin{Let's put a teaser. We can find examples like Fig. 4. There are 4 tasks: 1) text-guided, subject-driven, 2) text-guided, 3) subject-driven, 4) pure inpainting. Showcase our capability.}
Image inpainting can be viewed as a specialized form of image generation, where the goal is to generate content only for specific regions of a given image while keeping the rest unchanged. With the recent advancements in text-to-image synthesis models, the field of image inpainting has also experienced substantial improvements in terms of both quality and generalizability.

Texts and exemplar images are two common forms of conditions for image inpainting. Despite sharing identical objectives, these conditions lead to different requirements. In text-guided inpainting~\cite{}, the primary focus is on generating outputs faithful to the given texts, without specific demands on the appearance of the generated subject. This task emphasizes editability, requiring the model to be versatile enough to create arbitrary scenes and subjects based on textual descriptions. In contrast, exemplar-based inpainting~\cite{} prioritizes producing outputs that are faithful to the reference subject, focusing on identity preservation with minimal emphasis on editability. Due to their distinct natures, most current research tends to excel at either one condition, leaving the exploration of their combined potential largely untouched.

In this work, we introduce the task of \textit{\textbf{Text-Guided Subject-Driven Image Inpainting}}, whose objective is to inpaint a specific subject while allowing modifications of the subject. Conditioning on both texts and reference subjects allow users to to merge the creativity of text descriptions with the precision of exemplar-based approaches. By harnessing the strengths of both conditions, this task paves the way for more creative and fine-grained inpainting. However, given the inherent trade-off between identity preservation and editability, achieving a balance between these two contradictory objectives remains a formidable challenge.

To address the aforementioned issue, we devise a bottom-up approach that first computes dense subject features ensure accurate subject replication, and applies filtering to remove excessive subject details, encouraging editability. Specifically, we compute dense features using the UNet encoder of the pre-trained diffusion model. We then rank each token and retain only tokens with high scores. Our token selection module preserves essential tokens for identity preservation while avoiding direct subject copying.
%
Furthermore, to enhance text control, we propose a decoupling regularization during training. Instead of recovering only the masked region, we compute losses on the entire image, forcing network to leverage text captions for restoring details beyond the reference subject, preventing direct copying and significantly improving text-conditioning in the presence of reference subjects. Our experiments demonstrate that our method preserves identity more effectively and allows for more flexible text controls compared to existing state-of-the-art approaches. Our contributions are summarized as follows:

\begin{itemize}
    \item We introduce the text-guided subject-driven image inpainting task, a novel task that require balance between identity preservation and editability.
    \item We propose a discriminative token selection module and decoupling regularization to mitigate subject copying and enhance text-conditioning.
    \item  We conducted extensive experiments to demonstrate the effectiveness of our method. 
\end{itemize}

\kelvin{It could be a bit short. Will add details if necessary.}

% Recently, diffusion probabilistic models (DPMs) is gaining wide attention due to its superior performance over GAN. In particular, the pretrained text-to-image diffusion model, e.g., Stable Diffusion \cite{rombach2022high}, enables many interesting applications, such as video generation \cite{ho2022imagen,harvey2022flexible,mei2023vidm,esser2023structure,blattmann2023align,molad2023dreamix,wu2023tune,luo2023videofusion}, image editing \cite{kawar2023imagic,couairon2022diffedit,mokady2023null,nichol2021glide,hertz2022prompt}. 
% In particular, SmartBrush \cite{xie2023smartbrush} finetunes the stable diffusion with instance segmentation datasets and allows generates contents in the missing region according to the text prompt. Paint-by-Example \cite{yang2023paint} replaces the CLIP text embedding with the CLIP image embedding of reference image and thus supports image-guided inpainting.  Both methods have been shown to achieve superior performances in different tasks. However, in many real-world cases, it would be desirable if the missing region can be controlled through the text and image simultaneously. For instance, we may fill the missing region with the teddy bear in the reference image while changing the color according to the text prompt. We term such goal as subject-driven image inpainting.


% %Unlike GAN which requires adversarial training, DPMs adds noises on the images and train a UNet to recover the clean images and thus is known to be more stable. DPMs have been shown effective in different tasks, such as text-to-image generation \cite{ramesh2022hierarchical,saharia2022photorealistic,rombach2022high,ramesh2021zero}, 


% To achieve subject-driven image inpainting, a straightforward way would be finetuning the pretrained diffusion model following the single condition image inpainting approaches \cite{xie2023smartbrush,yang2023paint} and inject additional information.  For instance, we may follow the text-guided image inpainting model \cite{xie2023smartbrush} and inject the reference image together with the text embeddings. However, there are mainly two challenges: 1) \textbf{Identity Preservation}. If we use reference image as condition directly, the model will learn a trivial mapping and leads to copy-paste artifcats during inference \cite{yang2023paint}.  To address this problem, \cite{yang2023paint} proposes to constrain the information of reference image and only uses the CLIP  \cite{radford2021learning} class token to represent the image, which avoids the copy-paste problem. However, the CLIP class token is mainly trained for contrastive learning and may fail to capture the unique information about the object. As a consequence, it fails to preserve the important identity of the object in reference image. 2) \textbf{Text Control}. If we use the text class label of the reference image as text prompt and also feed the reference image, the model tends to utilize the reference image information directly and ignore the text condition. Consequently, the model fails to manipulate the object according to the text prompt during inference. 


% In this paper, we propose a novel approach that support subject-driven image inpainting while addressing above two important challenges.  Firstly, we choose to use the U-net downstack of the diffusion model to extract features of reference image since CLIP model tends to ignore the unique region of the images. Insteaf of feeding all tokens into the model, we proposes to rank each token by computing the pairwise distance. The score for each token is the summation of attentions from other tokens. If the token is specical (dissimilar to other tokens), the score is low. Then we rank the token in ascending order and only select the top tokens. In this way, the model learns to utilizes the unique regions of the reference object while avoiding copying the reference object since we only use part of them.  Secondly, we propose a decoupling regularization for enhancing text control for the inpainting task. We do not feed the coupled segmentation class label and segmentation object and we add noises on the whole image and uses the image caption and a random segmentation object to denoise the image. The model cannot ignore the text condtions otherwise it fails to denoise the other objects in the input image.  We evaluate our model on different datasets and show that our method learns to preserve much better identity than the state-of-the-art approaches and also enables flexible text controls. Our contributions can be summarized as follows:

% \begin{itemize}
%     \item We introduce the subject-driven image inpainting task and proposes a discriminative token selection module to preserve the identity of the reference object while avoiding copy-paste problem. 
%     \item We introduce a decoupling regularization to address the text control problem so the model allows generates the manipulated objects in the reference image according to the text prompt.
%     \item  We conducted experiments and user study. The quantitative and qualitative results demonstrate the effectiveness of our method. 
    
% \end{itemize}

%select discriminative tokens by computing the pairwise distance across tokens.  



%Subject driven image generation has been gaining wide attention 



%In this paper, we are 


%Recently, 
%it has been shown that inpainting with additional conditions can achieve impressive performance 
%inpainting or additional conditions, such as text or objects in the reference images \cite{xie2023smartbrush,yang2023paint}. 

